Entropy-Guided Attention for Private LLMs

The pervasiveness of proprietary language models has raised critical privacy concerns, necessitating advancements in private inference (PI), where computations are performed directly on encrypted data without revealing users' sensitive information. While PI offers a promising solution, its practical deployment is hindered by substantial communication and latency overheads, primarily stemming from nonlinear operations. To address this, we introduce an information-theoretic framework to characterize the role of nonlinearities in decoder-only language models, laying a principled foundation for optimizing transformer-architectures tailored to the demands of PI. By leveraging Shannon's entropy as a quantitative measure, we uncover the previously unexplored dual significance of nonlinearities: beyond ensuring training stability, they are crucial for maintaining attention head diversity. Specifically, we find that their removal triggers two critical failure modes: {\em entropy collapse} in deeper layers that destabilizes training, and {\em entropic overload} in earlier layers that leads to under-utilization of Multi-Head Attention's (MHA) representational capacity. We propose an entropy-guided attention mechanism paired with a novel entropy regularization technique to mitigate entropic overload. Additionally, we explore PI-friendly alternatives to layer normalization for preventing entropy collapse and stabilizing the training of LLMs with reduced-nonlinearities. Our study bridges the gap between information theory and architectural design, establishing entropy dynamics as a principled guide for developing efficient PI architectures. The code and implementation are available at https://github.com/Nandan91/entropy-guided-attention-llm

==> equations/entropy_And_temp_brief.tex <==

{\bf Setup}
Let \(\mathbf{A}^{(h,l)} \in \mathbb{R}^{T\times T} \) be the attention matrix of $h$-th head in $l$-th layer, where $T$ is context length. 
The elements of the attention matrix, \( a_{ij}^{(l, h)} \), represent the attention weights, which are non-negative and sum to one for each query position as follows:

\vspace{-1em}

\begin{equation}
\mathbf{A}^{(l, h)} = \left[ a_{ij}^{(l, h)} \right]_{T \times T}, \quad \text{where} \quad a_{ij}^{(l, h)} \geq 0 \quad \text{and} \quad \sum_{j=1}^{T} a_{ij}^{(l, h)} = 1
\end{equation}


This square matrix is generated by applying the softmax operation over the key length for each query position as follows (i.e., \(\mathbf{X} \in \mathbb{R}^{T\times T}\) \(\mathbf{X}_i \in \mathbb{R}^{1\times T}\) ): 

\vspace{-1.5em}

\begin{equation} 
\mathbf{A}^{(h,l)}(\mathbf{X}) = \text{Softmax}\Big(\frac{1}{\sqrt{d_k}} (\mathbf{X} \mathbf{W}^Q) (\mathbf{X}{\mathbf{W}^K})^\top \Big), \; \text{where} \quad \text{Softmax}(\mathbf{X}_i) = \frac{\exp \left(x_{i} \right)}{\sum_{j=1}^{T} \exp \left( x_{j} \right)}
\end{equation}


Thus, each element \( a_{ij}^{(l, h)} \) of the attention matrix can be represented as:

\vspace{-1em}

\begin{equation}
a_{ij}^{(l, h)} = \frac{\exp\left(\frac{1}{\sqrt{d_k}} (\mathbf{X}_i \mathbf{W}^Q) (\mathbf{X}_j \mathbf{W}^K)^\top \right)}{\sum_{k=1}^{T} \exp\left(\frac{1}{\sqrt{d_k}} (\mathbf{X}_i \mathbf{W}^Q) (\mathbf{X}_k \mathbf{W}^K)^\top \right)}
\end{equation}


{\bf Entropy of the Attention Matrix}
Entropy measures the uncertainty in a probability distribution, quantifying the information needed to describe a stochastic system's state \citep{shannon1948mathematical,jaynes1957information}. For a probability distribution \( P(x) \), the entropy is computed as \( \mathbf{E}(P) = -\sum_{x} P(x) \log P(x) \).

In softmax-based attention mechanisms, entropy evaluates the sharpness or spread of the softmax scores for each query position \citep{ghader2017does,vig2019analyzing}. Each softmax operation yields one entropy value. Higher entropy indicates a more uniform distribution of softmax scores over the key length, while lower entropy signifies a more focused distribution on certain features \citep{nahshan2024linear}.

To compute the entropy for one head, we average the entropy values across all query positions \citep{zhai2023stabilizing}. The entropy \( \mathbf{E}^{(l, h)} \) for the \( h \)-th head in the \( l \)-th layer of an attention matrix is given by:

\vspace{-1em}

\begin{equation}
\mathbf{E}^{(l, h)} = -\frac{1}{T} \sum_{i=1}^{T} \sum_{j=1}^{T} a_{ij}^{(l, h)} \log \left( a_{ij}^{(l, h)} + \epsilon \right)
\end{equation}
where \( \epsilon \) is a small constant added for numerical stability to prevent taking the log of zero. Further, we introduce a learnable temperature (\( t \in \mathbb{R}^{H \times T} \)) for each softmax operation in every head to adjust the sharpness of the attention scores. A higher temperature value (\( t > 1 \)) diffuses the attention scores and increases the entropy value, while a lower temperature value (\( t < 1 \)) sharpens the attention scores and reduces the entropy value (see Appendix). With the learnable temperature parameters, the attention matrix can be expressed as follows:

\vspace{-1.5em}

\begin{equation}
\mathbf{A}^{(l, h)}(t) = \left[ a_{ij}^{(l, h)}(t) \right]_{T \times T}, \quad \text{where} \quad a_{ij}^{(l, h)}(t) = \frac{\exp\left(\frac{1}{t_i \sqrt{d_k}} (\mathbf{X}_i \mathbf{W}^Q) (\mathbf{X}_j \mathbf{W}^K)^\top \right)}{\sum_{k=1}^{T} \exp\left(\frac{1}{t_i \sqrt{d_k}} (\mathbf{X}_i \mathbf{W}^Q) (\mathbf{X}_k \mathbf{W}^K)^\top \right)}
\end{equation}



\begin{equation}
\mathbf{A}^{(l, h)}(t) = \left[ a_{ij}^{(l, h)}(t) \right]_{T \times T},
\mathbf{E}^{(l, h)}(t) = -\frac{1}{T} \sum_{i=1}^{T} \sum_{j=1}^{T} a_{ij}^{(l, h)}(t) \log \left( a_{ij}^{(l, h)}(t) + \epsilon \right)
\end{equation}




\begin{algorithm}
\caption{Entropy Regularization Loss Computation}
\textbf{Inputs:} $\text{attentions}$: List of attention matrices, $\text{blocks}$: List of transformer blocks, $T$: Sequence length, $\lambda$: Hyper-parameter for Regularization loss weightage, $\gamma$: Hyper-parameter for  Tolerance margin \\
\textbf{Output:} $\mathcal{L}_{\text{total}}$: Total loss including entropy regularization
\begin{algorithmic}[1]
\State $\mathcal{L}_{\text{entropy}} \leftarrow 0$
\State $\text{E}_{\text{max}} \leftarrow \log(T)$ \Comment{Theoretical maximum value of entropy}
\State \(\text{Tol}_{\text{margin}} \leftarrow \gamma \text{E}_{\text{max}} \) \Comment{Tolerance margin is set as a small fraction of $\text{E}_{\text{max}}$}
%\State $H \leftarrow \text{block.attn.num\_heads}$ 
%\State $L \leftarrow \text{len(attentions)}$ 
\For{each layer $l$ in layers}
    \State $\mathcal{L}_{\text{layer}} \leftarrow 0$
    \State $\text{A}(t) \leftarrow \text{attentions}[l]$  \Comment{Attention matrix with learnable temperature for each query position}
    \State $\text{block} \leftarrow \text{blocks}[l]$
    \State $\theta^{(l, h)} \leftarrow \text{block.attn.reg\_th\_weights}$  \Comment{Learnable threshold weights for each head}
    \State $\text{E}^{(l,h)}(t) \leftarrow -\frac{1}{T} \sum_{i=1}^{T} \sum_{j=1}^{T} \text{A}_{ij}(t) \log(\text{A}_{ij}(t))$  \Comment{Calculate entropy for each head}
    \For{each head $h$ in heads}
        \State $\delta^{(l,h)} \leftarrow \text{E}^{(l,h)}(t) - \theta^{(l,h)} \text{E}_{\text{max}}$  \Comment{Deviation from head-specific threshold}
        \State $\text{penalty} \leftarrow (\delta^{(l,h)})^2 \mathbb{I}(|\delta^{(l,h)}| > \text{Tol}_{\text{margin}})$  \Comment{Penalize iff deviation exceeds Tolerance}
        \State $\mathcal{L}_{\text{layer}} \leftarrow \mathcal{L}_{\text{layer}} + \text{penalty}$
    \EndFor
    \State $\mathcal{L}_{\text{layer}} \leftarrow \frac{\mathcal{L}_{\text{layer}}}{\text{block.attn.num\_heads}}$  \Comment{Average over heads}
    \State $\mathcal{L}_{\text{entropy}} \leftarrow \mathcal{L}_{\text{entropy}} + \mathcal{L}_{\text{layer}}$
\EndFor
\State $\mathcal{L}_{\text{entropy}} \leftarrow \frac{\mathcal{L}_{\text{entropy}}}{\text{len(attentions)}}$  \Comment{Average over layers}
\State $\mathcal{L}_{\text{total}} \leftarrow \mathcal{L}_{\text{CE}} + \lambda \mathcal{L}_{\text{entropy}}$ \\
\Return $\mathcal{L}_{\text{total}}$
\end{algorithmic}
\end{algorithm}







==> figures/11_fig_recovered_collapse.tex <==


\begin{figure} [t]
\centering
\subfloat[Weight normalization in FFN]{\includegraphics[width=.33\textwidth]{plots/ent_layerwise_comparison_wnorm}} 
\subfloat[Spectral normalization in FFN]{\includegraphics[width=.33\textwidth]{plots/ent_layerwise_comparison_snorm}} 
\subfloat[Learnable scaling of FFN outputs]{\includegraphics[width=.33\textwidth]{plots/ent_layerwise_comparison_scaled_ffn}}   \vspace{-.8em}
\caption{Mitigating entropy collapse in the deeper layers of a softmax-only GPT-2 model by employing weight or spectral normalization in FFN, or by appropriately scaling FFN block outputs.} 
\label{fig:RecoveredEntCollapse}
\end{figure} 

==> figures/12_fig_learnable_neg_slope.tex <==



\begin{wrapfigure}[12]{r}{0.64\textwidth}
\centering
\vspace{-2\intextsep}
\subfloat[Layerwise learnable slope]{\includegraphics[width=.32\textwidth]{plots/layerwise_neg_slope}} 
\subfloat[Global learnable slope]{\includegraphics[width=.32\textwidth]{plots/neg_global_slope}} \vspace{-1em}
\caption{Learnable negative slope for leaky ReLU in the FFN of LN-free GPT-2. (a) Layerwise slopes and (b) global slope, both converge toward zero during training, indicating a preference for zero negative slope in LN-free architectures. } 
\label{fig:LearnableNegSlope}
\end{wrapfigure}




==> figures/1_fig_intro_gpt2.tex <==

\begin{figure} [htbp]
\centering
\includegraphics[width=.99\textwidth]{plots/latency_comm_ppl_gpt2_12L_CLen128} \vspace{-1em}
\caption{Latency and communication savings through nonlinearity and FLOPs reduction steps when AERO is applied on GPT-2,  and trained from scratch on CodeParrot dataset. Further, we benchmark AERO against the SOTA \cite{he2024simplifying} at iso-latency points. See Table \ref{tab:GPT2CLen128} for a detail analysis.} 
\label{fig:GPT2vsSOTA}
\end{figure} 


%Latency and communication savings through nonlinearity and FLOPs reduction steps when AERO is applied on Pythia-70M, and model is trained from scratch on %CodeParrot dataset with context length 256. Further, we benchmark AERO against the SOTA \cite{he2024simplifying} at iso-latency points.

==> figures/6_fig_entropic_overlaod_solved.tex <==

\begin{wrapfigure}[14]{r}{0.55\textwidth - .95\columnsep}
\centering
\vspace{-1\intextsep}
\includegraphics[scale=0.18]{plots/entropy_bins_mlpgains} 
\vspace{-.8em}
\caption{While normalizing weights or scaling outputs in the FFN of Softmax-only (GPT-2) model prevents entropy collapse, our proposed entropy regularization effectively mitigates  entropic overload.} 
\label{fig:EntropicOverlaodSolved}
\end{wrapfigure}

==> figures/7_fig_layerwise_perplexity_lf_dr.tex <==
\begin{figure}[t] \centering
\includegraphics[width=.49\textwidth]{plots/perplexity_comparison_ffn_lf_dr} \vspace{-2em}
\caption{Perplexity analysis for progressive FFN complexity reduction when GELUs are dropped from all but one layer in GPT-2. Perplexity largely remains unaffected when linear layers are combined and then substituted with an identity connection, compared to SlimGELU FFN, suggesting the redundancy of linear layers in FFN when GELU activation layers are eliminated. }
\label{fig:LayerwisePerplexLfDr}
\end{figure}

%The findings indicate that complexity remains relatively stable even when linear layers are combined and then substituted with an identity link, as seen in comparison to the SlimGELU FFN, highlighting resilience to these particular structural changes.  

==> figures/9_fig_softmax_nan.tex <==


%\begin{figure} [htbp]
%\centering
%\subfloat[Layerwise NaNs]{\includegraphics[width=.49\textwidth]{plots/layerwise_NaNs}} 
%\subfloat[Scaled FFN entropy]{\includegraphics[width=.49\textwidth]{plots/entropy_hmap_SM_mlp_gains}} \\ 
%\subfloat[Value of learnable scaling factors]{\includegraphics[width=.49\textwidth]{plots/inverse_mlp_block_resid_gain}} 
%\subfloat[Value of learnable  skip scaling factors]{\includegraphics[width=.49\textwidth]{plots/inverse_mlp_block_skip_gain}}  
%\caption{Patterns for Softmax-only GPT-2 model} 
%\label{fig:SoftmaxNaN}
%\end{figure} 

\begin{wrapfigure}[11]{r}{0.65\textwidth - .85\columnsep}
\centering
\vspace{-2\intextsep}
\subfloat[Layerwise NaNs \label{subfig:LayerwiseNaNs}]{\includegraphics[width=.32\textwidth]{plots/layerwise_NaNs}} 
\subfloat[ Entropy heatmap \label{subfig:EntHmapSM}]{\includegraphics[width=.33\textwidth]{plots/ent_hmap_no_ln_no_act}} 
\vspace{-1em}
\caption{Training collapses in softmax-only GPT-2 model.} 
\label{fig:SoftmaxNaN}
\end{wrapfigure}

==> tables/11_table_pythia_70M_clen_256.tex <==



\begin{table}[t]
\centering
\caption{Results, and comparison against SOTA \citep{he2024simplifying}, when  Pythia-70M ($L$=6, $H$=8, $d$=512) \citep{biderman2023pythia} model is trained from scratch on CodeParrot dataset \citep{codeParrot} with context length  256.}
\label{tab:Pythia70M}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{p{0.2cm}lclcccccc}
\toprule
& \multirow{2}[4]{*}{Network Arch.} & \multirow{2}[4]{*}{PPL} & \multirow{2}[4]{*}{\#Nonlinear Ops} & \multicolumn{2}{c}{\#FLOPs} & \multirow{2}[4]{*}{\shortstack{Comm.\\(GB)}} & \multirow{2}[4]{*}{\shortstack{Lat.\\(min.)}} & \multicolumn{2}{c}{Savings} \\
\cmidrule(lr){5-6} \cmidrule(lr){9-10}
& & & & FFN & Attn. & & & Comm. & Lat. \\
\midrule
\multirow{6}{*}{  \rotatebox[origin=c]{90}{Baseline} } & \multirow{3}{*}{${\tt SM + LN + G}$} & \multirow{3}{*}{2.69} & SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{3}{*}{14.5B} & \multirow{3}{*}{7.7B} & \multirow{3}{*}{25.32} & \multirow{3}{*}{8.21} & \multirow{3}{*}{1$\times$} & \multirow{3}{*}{1$\times$} \\
& & & LN:$24\times\mathbb{R}^{128\times768}$ & & & & & & \\
& & & G:$12\times\mathbb{R}^{128\times3072}$ & & & & & & \\ \cline{2-10}
& \multirow{3}{*}{${\tt SM + LN + R}$} & \multirow{3}{*}{2.76} & SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{3}{*}{14.5B} & \multirow{3}{*}{7.7B} & \multirow{3}{*}{9.44} & \multirow{3}{*}{6.06} & \multirow{3}{*}{2.68$\times$} & \multirow{3}{*}{1.35$\times$} \\
& & & LN:$24\times\mathbb{R}^{128\times768}$ & & & & & & \\
& & & R:$12\times\mathbb{R}^{128\times3072}$ & & & & & & \\
\midrule
\multirow{6}{*}{  \rotatebox[origin=c]{90}{SOTA \citep{he2024simplifying}} } & \multirow{2}{*}{${\tt SM + ScFFN}$} & \multirow{2}{*}{4.00} &  SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{2}{*}{14.5B} & \multirow{2}{*}{3.9B}  & \multirow{2}{*}{6.83} & \multirow{2}{*}{5.31} &  \multirow{2}{*}{3.71$\times$} & \multirow{2}{*}{1.55$\times$} \\
& & & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\ \cline{2-10}
&\multirow{2}{*}{${\tt SM + ScFuFFN}$}  & \multirow{2}{*}{3.97} &  SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{2}{*}{1.8B} & \multirow{2}{*}{3.9B}  & \multirow{2}{*}{6.31} & \multirow{2}{*}{4.50}  & \multirow{2}{*}{4.00$\times$} & \multirow{2}{*}{1.82$\times$}\\
& & & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\ \cline{2-10}
&\multirow{2}{*}{${\tt SM + ScFuFFNi_1}$}  & \multirow{2}{*}{4.00} &  SM:$144\times\mathbb{R}^{128\times128}$ & \multirow{2}{*}{1.2B} & \multirow{2}{*}{3.9B}  & \multirow{2}{*}{6.30} & \multirow{2}{*}{4.44} & \multirow{2}{*}{4.00$\times$}  & \multirow{2}{*}{1.85$\times$} \\
& & & LN: $1\times\mathbb{R}^{128\times768}$ & & & & & & \\
\midrule
\multirow{5}{*}{  \rotatebox[origin=c]{90}{\bf AERO} } &${\tt SM + ScFFN}$ & 3.50 &  SM:$144\times\mathbb{R}^{128\times128}$ & 14.5B & 7.7B &  6.95 & 5.68  & 3.64$\times$ & 1.45$\times$ \\			
&${\tt SM + ScFuFFN}$ & 3.48 &  SM:$144\times\mathbb{R}^{128\times128}$ & 1.8B & 7.7B & 6.43 & 4.76  & 3.94$\times$  & 1.72$\times$ \\
&${\tt SM + ScFuFFNi_6}$ & 3.54 & SM:$144\times\mathbb{R}^{128\times128}$ & 0.9B & 7.7B  & 6.29 & 4.23  & 4.00$\times$ & 1.94$\times$ \\ \cline{2-10}
&$\text{EReg}({\tt SM(t) + ScFuFFN})$ & 3.21 &  SM:$144\times\mathbb{R}^{128\times128}$ & 1.8B & 7.7B  & 6.43 & 4.76  & 3.94$\times$ & 1.72$\times$ \\
&$\text{EReg}({\tt SM(t) + ScFuFFNi_6})$ & 3.25 & SM:$144\times\mathbb{R}^{128\times128}$ & 0.9B & 7.7B &  6.29 & 4.23 & 4.00$\times$ & 1.94$\times$ \\
\bottomrule
\end{tabular}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%


	






==> tables/12_table_pythia_70M_dissipating_nonlinearity.tex <==

\begin{table}[htbp]
\caption{Results for nonlinearity reduction in Pythia-70M ($L$=6, $H$=8, $d$=512) on CodeParrot dataset. LN-free architecture with ReLU activations in FFN (i.e., ${\tt SM+R}$) significantly outperform their GELU counterpart (i.e., ${\tt SM+G}$) across various content length ($T$). }
\label{tab:PythiaDissipatingNonlin}
\centering
\begin{tabular}{lcccc} \toprule
& \multicolumn{2}{c}{$T$=128} & \multicolumn{2}{c}{$T$=256} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& Eval PPL &+$\Delta$(\%) & Eval PPL & +$\Delta$(\%) \\ \toprule
SM+LN+G & 3.512 & 0.00 & 3.054 & 0.00 \\
SM+LN+R & 3.590 & 2.22 & 3.107 & 1.73 \\
SM+LN & 4.445 & 26.56 & 3.836 & 25.60 \\
SM+G & 4.086 & 16.35 & 3.570 & 16.87 \\
SM+R & 3.736 & 6.36 & 3.273 & 7.17 \\
\bottomrule
\end{tabular} 
\end{table}

















==> tables/1_table_related_work.tex <==

\begin{table} [t]
\caption{Comparison}
\label{tab:PreviousWork}
\centering 
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{cclcccccc} \toprule
\multirow{2}{*}{ Approach } & \multirow{2}{*}{ Arch. } & \multirow{2}{*}{ \shortstack{Crypto \\ Setting} } & \multicolumn{4}{c}{Optimized Component} & \multirow{2}{*}{ Granularity } & \multirow{2}{*}{\shortstack{Train from\\scratch }}\\ 
\cmidrule(lr{0.5em}){4-7}
& & & LN & GELU & Softmax & FLOPs & &\\ \toprule
THE-X \cite{chen2022x} & BERT & 2pc (HE) & & & & & & \ding{55}\\
Iron \cite{hao2022iron} & BERT & 2pc (HE + MPC) & & & & & & \ding{55} \\
MPCFormer  \cite{li2023mpcformer} & BERT & 3pc (MPC) & & & & & & \ding{55} \\
MPCViT \cite{zeng2022mpcvit} & ViT & 2pc (HE + MPC)& & & & & & \ding{55} \\
Sal-ViT \cite{Zhang_2023_ICCV} & ViT & 3pc (MPC) & & & & & & \ding{55} \\
RNA-ViT \cite{chen2023rna} & ViT & 3pc (MPC) & & & & & & \ding{55} \\
PriViT \cite{dhyani2023privit} & ViT & 2pc (HE + MPC) & & & & & & \ding{55}\\
Primer \cite{zheng2023primer} & BERT & 2pc (HE + MPC)  & & & & & & \ding{55}\\
Privformer \cite{akimoto2023privformer} & Transformer & 3PC (MPC) & & & & & & \ding{55} \\
Zimerman et al. \cite{zimerman2023converting} & BERT,ViT & 2pc (HE) & & & & & & \ding{55} \\ 
AERO ({\bf Ours}) & GPT-2 & 2pc (HE + MPC) & \checkmark & \checkmark & & \checkmark & Network & \checkmark \\ \bottomrule
%CipherGPT \cite{hou2023ciphergpt} & GPT-2 & 2pc (HE + MPC) & & & & & & \\
%Bumblebee \cite{lu2023bumblebee} & BERT, GPT-2, ViT& 2pc (HE + MPC) & & & & & & \\
%BOLT \cite{pang2023bolt} & GPT2 & 2pc & & & & & & \\
%PUMA \cite{dong2023puma} & LLaMA & 3PC & & & & & & \\
%SIGMA \cite{gupta2023sigma} & GPT2 & 3PC & & & & & & \\bottomrule
\end{tabular} }
\end{table}


==> tables/3_table_ffn_lf_dr.tex <==

\begin{table}[t]
\centering
\caption{Perplexity  analysis for understanding the impact of dropping  GELUs from all FFN layers, and subsequent complexity reduction through layer fusion and then substituting them with an identity connection. An 3.2$\times$ FLOPs reduction is achieved, at the cost of a 24\% increase in perplexity, compared to standard GPT-2 model with GELUs in their FFNs. }
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{ccccccc} \toprule 
\multirow{2}{*}{ GPT-2 configuration } & \multirow{2}{*}{GELUs} & \multirow{2}{*}{Params} & \multirow{2}{*}{FLOPs} & \multirow{2}{*}{Perplexity} & \multicolumn{2}{c}{Savings} \\
\cmidrule(lr{0.5em}){6-7} 
& & & & & Params & FLOPs \\ \toprule 
Baseline  & 4.72M & 124.2M & 10.6B & 2.69 & 1.0$\times$ & 1.0$\times$ \\
SlimGELU FFN & 0 &124.2M & 10.6B & 3.38 & 1.0$\times$ & 1.0$\times$ \\
FusedLayer FFN & 0  &74.7M & 5.1B & 3.34 & 1.7$\times$ & 2.1$\times$ \\
IdentityLink FFN & 0  &67.6M & 3.3B & 3.33 & 1.8$\times$ & 3.2$\times$ \\ \bottomrule 
\end{tabular} }
\end{table}



